Expanding Boundaries: Cross-Media Routing for Seamless Underwater and Aerial Communication

The colossal evolution of wireless communication technologies over the past few years has driven increased interest in its integration in a variety of less-explored environments, such as the underwater medium. In this magazine paper, we present a comprehensive discussion on a novel concept of routing protocol known as cross-media routing, incorporating the marine and aerial interfaces. In this regard, we discuss the limitation of single-media routing and advocate the need for cross-media routing along with the current status of research development in this direction. To this end, we also propose a novel cross-media routing protocol known as bubble routing for autonomous marine systems where different sets of AUVs, USVs, and airborne nodes are considered for the routing problem. We evaluate the performance of the proposed routing protocol by using the two key performance metrics, i.e., packet delivery ratio (PDR) and end-to-end delay. Moreover, we delve into the challenges encountered in cross-media routing, unveiling exciting opportunities for future research and innovation. As wireless communication expands its horizons to encompass the underwater and aerial domains, understanding and addressing these challenges will pave the way for enhanced cross-media communication and exploration.

==> Old_files/abstract.tex <==
\begin{abstract} 

In this preliminary work, we provide a novel physical layer authentication mechanism in underwater acoustic communication networks. Specifically, we propose position of the transmitter nodes for authentication purpose. First, we do position estimation from the received signals at the anchored/reference nodes deployed at the fixed positions in a predefined  underwater region based on Time of Arrival (ToA) estimation. We also derive the distribution of inherent uncertainty in the estimation. Next, on the estimated position, we do binary hypothesis testing to decide for the legitimacy of the transmitter nodes. We provide closed form expressions of false alarm and missed detection resulted from binary hypothesis testing. We provide the simulation results demonstrating errors' behaviour against total transmit power.
\end{abstract}


==> Old_files/allsec.tex <==
\section{Introduction}
\label{sec:intro}

Underwater acoustic communication has gained a significant attention due to its promising applications in marine life exploration, natural resources finding, underwater navigation and military operations\cite{song2019editorial}. A plethora of research has been reported in the recent past covering the aspects of modem designs to signal processing techniques of underwater acoustic communication \cite{fattah2020survey}.  The broadcast nature of underwater acoustic communication makes the networks vulnerable to many types of malicious attacks. With passage of time, different attacks were studied with different counter mechanisms \cite{aman2022security}. One of the prominent attacks is the spoofing/impersonation attack, where a malicious node aims to mimic one of the legitimate nodes of the network in order to get access and destroy the integrity of the system  \cite{Ammar:VTC:2017}, \cite{waqas:Sensors:2021}. To counter such attacks, recently, the idea of physical layer authentication is explored for underwater acoustic communication networks \cite{Waqas:Access:2018,xiao2018learning,khalid2020physical,9676618}, where a physical layer feature serves as device fingerprint (can be thought as authentication key). In this regard, we report our investigation on the use of distance and angle of arrival as device finger prints for physical layer authentication, where closed form expressions for error probabilities are derived \cite{Waqas:Access:2018}. Next, \cite{xiao2018learning} study power delay profile of underwater acoustic channel using deep reinforcement learning approach to detect impersonation. Following our work, authors in \cite{khalid2020physical} report two angles of arrival (azimuth and elevation) to counter impersonation in line of sight underwater acoustic communication. Recently, authors in \cite{9676618}  report time reversal resonating strength based physical layer authentication in underwater acoustic sensor networks.

In this work, for the first time, we study position of transmitting node as device fingerprint to decide for impersonation attacks at the physical layer. The detailed contributions of this paper are given below:
\begin{itemize}
    \item We used Time of Arrival (ToA) based localization to extract the coordinates of transmitting node. For this purpose, we exploit our previously proposed best unbiased estimator for ToA estimation. At the end, we find the distribution of the inherit uncertainty in the estimation process.
    
    \item Next, We build a test statistic for binary hypothesis testing in order to decide whether the estimated position belongs to legitimate node or malicious. We derive the distributions of conditional events (i.e., test statistic given legitimate or malicious transmissions) and provide closed form expressions for the two error probabilities (i.e., false alarm and missed detection).
    
\end{itemize}






{\bf Outline.} The rest of this paper is organized as follows. Section \ref{sec:sys-model} presents system model, Section \ref{sec:methods} provides the proposed physical layer authentication mechanism, Section \ref{sec:results}  discusses the simulation results and  Section \ref{sec:conclusion} concludes the paper.
\section{System model}
\label{sec:sys-model}

We consider static two nodes setup (i.e., legitimate Autonomous Underwater Vehicle (AUV) and a malicious AUV) with three anchored/reference nodes, which are used to estimate the position of transmitter AUVs, as shown in Fig. \ref{fig:sysmodel}. We assume that the anchored nodes are perfectly synchronized and connected to ground station/surface ship via secured channel. We consider a one-way authentication system. Specifically, the considered malicious AUV is an intruder which sends malicious packets to the system from time to time while trying to impersonate legitimate AUV. Therefore, a systematic framework is needed to authenticate the sender of every packet it receives. This way, ground station  can reject packets from malicious node. We consider range-based localization technique (i.e., Time-of-Arrival (ToA)) to extract position coordinates from the received signals at the reference nodes. 



We assume that the one-way authentication channel in Fig. \ref{fig:sysmodel} is time-slotted. That is, packets arrive at reference nodes at discrete-time instants $t_m$ where $t_m-t_{m-1}=T$ is the time-gap between two successively received packets at reference nodes. Moreover, each received packet is $T_p < T$ seconds long. 

\begin{figure}[ht]
\begin{center}
	%\includegraphics[width=8cm,height=7cm]{Figures/SM.pdf} 
	\includegraphics[width=8cm,height=7cm]{Figures/post_authen.PNG} 
\caption{System Model}
\label{fig:sysmodel}
\end{center}
\end{figure}

\section{Proposed PHY layer authentication framework}
\label{sec:methods}

\subsection{Position estimation}
\subsubsection{Distance Estimation}
Let $t_i$ is the arrival time of a signal (ToA) at the $i$-th reference node. We exploit our previous work \cite{Waqas:Access:2018} to estimate ToA of the transmitter nodes  in the presence of heavily frequency dependent pathloss and colored nose using best unbiased estimator (i.e., meeting Crammer Rao bound (CRB)). Specifically, the distance of transmitter node from $i-$th anchored node is estimated using distance equation, given below:
\begin{align}
\hat{d_i}=c\hat{t}_i    
\end{align} 
where $c$ is the speed of sound in water, $\hat{t}_i \sim N(t_i,\hat{\sigma}_i^2)$ is the estimated ToA with $t_i$ is the actual time of arrival and $\sigma_i^2$ is the variance of the best unbiased estimator \cite{Waqas:Access:2018}, which can be expressed as \cite{Waqas:Access:2018}: 
\begin{align}
    \hat{\sigma}_i^2 =  \frac{ PL_i(f)}{4P\mathbf{\Hat{s}^TC^{-1}\Hat{s}}},
\end{align}
where $P$ is the transmit power, $c$ is the underwater speed of sound, \mathbf{C} is the covariance matrix of colored noise. $\mathbf{\Hat{s}}$ is the partial derivative of pseudo random sequence $\mathbf{s}$\footnote{A random sequence or message a transmitter needs to transmit for ToA estimation \cite{Waqas:Access:2018} at the anchored nodes.}. The estimated distance can be written as: $\hat{d}_i^2=d_i+n_i$, where
where $\hat{d_i}$ is the estimated distance, $d_i$ is the true distance of transmitter to the $i$-th anchored node, $n_i\sim N(0,\sigma^2)$  is the uncertainty/noise in the estimator with variance $\sigma^2= \frac{c^2 PL_i(f)}{4P\mathbf{\Hat{s}^TC^{-1}\Hat{s}}}$. The pathloss $PL_i(f)$ of a transmitter to $i$-th anchored node is given as \cite{stojanovic2007relationship}:
\begin{align}
    PL_i(f)_{[dB]}= \nu 10\log_{10}(d)+d\alpha(f)_{[dB]},
\end{align}
where $d\alpha(f)_{[dB]}=\frac{0.11f^2}{1+f^2}+\frac{44f^2}{4100+f^2}+2.75\times 10^{-4}f^2+0.003$ with $f$ as operating frequency.
\subsubsection{Coordinates Extraction}
Using the definition of the standard Euclidean distance, $d_i$ can be written as
\begin{align}
d_i^2=(x-x_i)^2+(y-y_i)^2    
\end{align}
Assuming high SNR regime we can write $\hat{d_i}^2\approx(d_i+n_i)^2=d_i^2+2n_id_i$.
Now  $\hat{d_i}^2$ can be expressed as
\begin{align}
\hat{d_i}^2=(x-x_i)^2+(y-y_i)^2+2n_i((x-x_i)^2+(y-y_i)^2)^2    
\end{align}
Now for all ''$i_s$'' the equation set resulted from the above equation can be written in matrix-vector form as
\begin{align}
AX+N=b
\end{align}
where 
\begin{align}
A=-2
\begin{bmatrix}
    x_1 & y_1 & -0.5   \\
    . & . & .   \\
     . & . & .  \\
    x_L & y_L & -0.5      
  \end{bmatrix} ,  N=2
  \begin{bmatrix}
    n_1d_1   \\
    .    \\
    . \\
     n_Ld_L     
  \end{bmatrix}, \nonumber \\ X=\begin{bmatrix} 
    x   \\
    y  \\
     x^2+y^2     
  \end{bmatrix} 
\ and 
\ b=\begin{bmatrix}
      \hat{d_1}^2-x_1^2-y_1^2 \\
    .   \\
     .\\
       \hat{d_L}^2-x_L^2-y_L^2   
  \end{bmatrix} \nonumber 
\end{align}
we can verify that $E[N]=0$, therefore above can be approximated as 
\begin{align}
\label{eq:aprox}
AX\approx b
\end{align}
now Eq. \ref{eq:aprox} is a least square problem, the solution to $S$ can be obtained as
\begin{align}
\label{eq:LS}
&\min_{X}\Vert b-AX \Vert_2^2\\
&=\min_X(b-AX)^T(b-AX) \nonumber
\end{align}
one can verify that Eq. \ref{eq:LS} is a convex function. To find the minimum we take the gradient $\nabla_X$ and equate it to zero gives us
 \begin{align}
X=(A^TA)^{-1}A^Tb
\end{align}
where $(A^TA)^{-1}A^T=A^{\dagger}$ also known as pseudo inverse of $A$.
Now, we are only interested in $x$ and $y$ components of $X$. so, the desired vector can be written as
\begin{align}
\hat{X}=[X(1) \ X(2)]^T
\end{align}
Next, we derive the distribution of $\hat{X}$, we can write Eq. () as:
From here we avoid to use the index $k$ for simplicity,
As $A^{\dagger}$ is a $3*L$ dimension matrix and we know that our desired component of $X$ lies in $\hat{X}$. Now let $\hat{A^{\dagger}}=A_{2*L}^{\dagger}$, then (7) can also be written as
\begin{align}
\hat{X}=\hat{A^{\dagger}}b
\end{align}
Or more precisely
\begin{align}
\hat{X}=\underbrace{\hat{A^{\dagger}}\begin{bmatrix}
      {d_1}^2-x_1^2-y_1^2 \\
    .   \\
     .\\
       {d_L}^2-x_L^2-y_L^2   
  \end{bmatrix}}_{True \ Co-ordinates} + \underbrace{2\hat{A^{\dagger}}\begin{bmatrix}
      n_1d_1\\
    .   \\
     .\\
       n_Ld_L   
  \end{bmatrix}}_{Noise}
\end{align} 

%\subsection{Kalman Filter}
%The state space equation of Kalman filter can be expressed as

\subsection{Hypothesis Testing}
 Let $\hat{
 X}_A$ the actual coordinates vector of Alice and $\hat{
 X}_E$ of Eve. $\text{H}_0$ is the hypothesis (also known as Null hypothesis) that Alice is the transmitter while $H_1$ is the hypothesis (also known as alternate hypothesis) that Eve is the transmitter  then we define test statistics as:
 
 \begin{align}
    \text{TS}=\Vert (\hat{A^{\dagger}}^T\hat{A^{\dagger}})^{-1}\hat{A^{\dagger}}^T\left( \hat{X}-\hat{
 X}_A \right)\Vert_2^2.
 \end{align}
Now, Binary hypothesis test can be defined as 
\begin{equation}
	\label{eq:H0H1}
	 \begin{cases} \text{H}_0 (\text{no impersonation}): & \text{TS}=\Vert \hat{A^{\dagger\dagger}}\left( \hat{X}-\hat{
 X}_A \right) \Vert_2^2. < \epsilon_{th} \\ 
                   H_1 (\text{impersonation}): & \text{TS}=\Vert \hat{A^{\dagger\dagger}} \left( \hat{X}-\hat{
 X}_A \right) \Vert_2. > \epsilon_{th} \end{cases}
\end{equation}
where $\hat{A^{\dagger\dagger}}=(\hat{A^{\dagger}}^T\hat{A^{\dagger}})^{-1}\hat{A^{\dagger}}^T$, $\epsilon_{th}$ is a predefined threshold. 
Equivalently, we have:
\begin{align} 
\label{eq:bht}
\text{TS} \gtrless_{\text{H}_0}^{H_1} {\epsilon_{th}}.
\end{align}
At this stage, we need to find the error probabilities (i.e., false alarm and missed detection). False alarm can be defined as the probability that BHT decides legitimate node as malicious node while missed detection is the probability that BHT decides malicious node as legitimate node. The false alarm $P_{fa}$ can be expressed as:
\begin{align}
    P_{fa}=Pr(\text{TS} \mid \text{H}_0 > \epsilon_{th})
\end{align}
To compute the above probability we need to find the distribution of the conditional event $\text{TS} \mid \text{H}_0$, which can be expressed as
\begin{align}
\label{eq:ts_H_0}
    \text{TS} \mid \text{H}_0&=\Vert \hat{A^{\dagger\dagger}}\left(\hat{
 X}_A+\mathbf{n}_A-\hat{
 X}_A\right) \Vert_2^2=\Vert \hat{A^{\dagger\dagger}} \mathbf{n}_A\Vert_2^2 \\
 &=4\left( (d_1^An_1^A)^2+(d_2^An_2^A)^2+...+(d_L^An_L^A)^2 \right) \nonumber \\
 &= \sum_{i=1}^L (2 d_i^An_i^A)^2 = \sum_{i=1}^L  (\hat{n}_i^A)^2  \nonumber
\end{align}
where $\mathbf{n}_A={2\hat{A^{\dagger}}\begin{bmatrix}
      n_1^Ad_1^A \
    .   \
     . \
       n_L^Ad_L^A   
  \end{bmatrix}} ^T$ with $d_i^A$ where $i \in \{1...L\}$ denotes the distance of legitimate node from $i$-th reference node and $\hat{n}_i^A \sim N(0,4(d_i^A)^2\sigma^2_i), \forall i$.  We can write $(2d_i^An_i^A)^2\sim \Gamma(1/2, 8(d_i^A)^2\sigma_i^2)$.
  So, the probability of false alarm is given as \cite{ansari2017new}:
  
  \begin{align}
    P_{fa}  =\sqrt{1/2} \prod_{i=1}^L \sqrt{\frac{1}{\kappa_i}} \ H_{L+1,L+1}^{0,L+1} \left[ e^{\epsilon_{th}} \mid \begin{matrix}
\Xi_L^1, (1,1,1)\\
\Xi_L^2, (0,1,1)
\end{matrix} \right],
  \end{align}
  where $\kappa_i=8(d_i)^2\sigma_i^2$, $ H_{.,.}^{.,.}$ is Fox-H function, $\Xi_L^1$ and $\Xi_L^2$ represent the bracket terms as: $\Xi_L^1= (1-\frac{0.5}{8(d_1^A)^2\sigma_1^2},1,0.5),...(1-\frac{0.5}{8(d_L^A)^2\sigma_L^2},1,0.5)$, $\Xi_L^2= (-\frac{0.5}{8(d_1^A)^2\sigma_1^2},1,0.5),...(-\frac{0.5}{8(d_L^A)^2\sigma_L^2},1,0.5)$.
  
  Now, to find the probability of missed detection, we need to find $\text{TS} \mid H_1$, which can be expressed as 
  \begin{align}
      \text{TS} \mid H_1&=\Vert \hat{A^{\dagger\dagger}}\left(\hat{
 X}_E+\mathbf{n_E}-\hat{
 X}_A\right) \Vert_2^2=\Vert \hat{A^{\dagger\dagger}} \mathbf{n_E}+\mathbf{d_{EA}}\Vert_2^2 \\
 &=4( (d_1^En_1+(d_1^E)^2-(d_1^A)^2)^2+... \nonumber \\ &..+((d_L^En_L)+(d_L^E)^2-(d_L^A))^2)
 = \sum_{i=1}^L (2 d_in_i)^2,  \nonumber
  \end{align}
  where $\mathbf{n}_E={2\hat{A^{\dagger}}\begin{bmatrix}
      n_1^Ed_1^E \
    .   \
     . \
       n_L^Ed_L^E   
  \end{bmatrix}} ^T$ with $d_i^E$ where $i \in \{1...L\}$ denotes the distance of malicious node from $i$-th reference node, $\hat{n}_i^E \sim N(0,4(d_i^E)^2\sigma^2_i), \forall i$ and $\mathbf{d_{EA}}={\begin{bmatrix}
      (d_1^E)^2-(d_1^A)^2 \
    .   \
     . \
      (d_L^E)^2-(d_L^A)^2  
  \end{bmatrix}} ^T$.
  Now, probability of missed detection can be expressed as \cite{castano2005distribution}:
  
 \begin{align}
     P_{md}= \frac{e^{-\frac{\epsilon_{th}}{2\beta}}}{(2\beta)^{\frac{L}{2}}} \frac{\epsilon_{th}^{\frac{L}{2}}}{\Gamma (\frac{L}{2}+1)} \sum_{k\geq 0} \frac{k!\zeta_k}{(\frac{L}{2}+1)_k}\mathbf{L}_k^{\frac{L}{2}}(\frac{(L+2)\epsilon_{th}}{4\beta \mu_0}),
 \end{align}
  with $\beta >0$, $\mu_0 >0$, $\zeta_k=\frac{\sum_{j=0}^{k-1} \zeta_j \xi_{k-j}}{k}$, \\ $\zeta_0=2(\frac{L}{2}+1)^{\frac{L}{2}+1}\exp{-\frac{1}{2}\sum_{i=1}^L \frac{\lambda_i \gamma_i (\frac{L}{2}+1-\mu_0)}{\beta \mu_0+\gamma_i (\frac{L}{2}+1-\mu_0)}} \bullet\frac{\beta^{\frac{L}{2}+1}}{\frac{L}{2}+1-\mu_0)}\prod_{i=1}^L (\beta \mu_0+\gamma_i (\frac{L}{2}+1-\mu_0))^{-\frac{1}{2}}$, \\
  $\xi_j=-\frac{j\beta(\frac{L}{2}+1)}{2\mu_0}\sum_{i=1}^L \lambda_i \gamma_i(\beta-\gamma_i)^{j-1} (\frac{\mu_0}{(\beta \mu_0+\gamma_i (\frac{L}{2}+1-\mu_0))})^{j+1}+(\frac{-\mu_0}{\frac{L}{2}+1-\mu_0})^j+\frac{1}{2}(\frac{\mu_0(\beta-\gamma_i)}{(\beta \mu_0+\gamma_i (\frac{L}{2}+1-\mu_0))})^{j+1}$, $\lambda_i=\frac{(d_1^E)^2-(d_1^A)^2}{\sigma_i}$, $\gamma_i=4(d_i^E)^2\sigma_i$, $\Gamma(.)$ indicates gamma function, $\mathbf{L}_k^{.}$ is the $k$-th  generalized Laguerre polynomial. 


\section{Simulation results}
\label{sec:results}
We use Python for simulations. We consider a rectangular area of $1000\times1000$ m$^2$, $L=3$ total number of anchored nodes with positions $[0,500]$, $[-500,-500]$, $[-500,500]$, legitimate AUV is fixed at origin (i.e., $X_A=[0,0]$ and position of malicious AUV is uniformly distributed. Further, we set center frequency $f=10$KHz, speed of sound $c=1500$m/s and spreading factor $\nu=1.5$. 

We choose transmit power $P$ (in dB Pascal (pa)) as controlled parameter or independent variable\footnote{Typically, the inverse of estimator variance is chosen as independent variable in the literature but as we can see that this parameter is different for different transmitters and anchored nodes. Therefore, we need a common parameter for fair comparison. } to generate the figures. We sweep $P$ from $0$ to $100$ dB pa because of its adoption  in the literature for underwater acoustic transmitters \cite{stojanovic2007relationship}.
\begin{figure}
\begin{center}
	%\includegraphics[width=8cm,height=7cm]{Figures/SM.pdf} 
	\includegraphics[width=8cm,height=6cm]{Figures/fa.png} 
\caption{Probability of false alarm $P_{fa}$ against the total transmit power $P$ in dB pa}
\label{fig:fa}
\end{center}
\end{figure}
Fig. \ref{fig:fa} demonstrates the trend of false alarm resulted from binary hypothesis testing Eq. \ref{eq:bht} with increase in the transmit power lowers the false alarm. This is due to the fact that increase in $P$ shrinks the variances $\sigma_i^2$ of the estimator  which makes the estimated distances close to the actual distances. On the other hand, the increase in the threshold $\epsilon_{th}$ produces low false alarm but it has a affect on missed detection.
\begin{figure}[ht]
\begin{center}
	%\includegraphics[width=8cm,height=7cm]{Figures/SM.pdf} 
	\includegraphics[width=8cm,height=6cm]{Figures/md.png} 
\caption{Probability of missed detection $P_{md}$ against the total transmit power $P$ in dB pa}
\label{fig:md}
\end{center}
\end{figure}
Fig. \ref{fig:md} demonstrates the behaviour of missed detection. We observe that missed detection $P_{md}$ decreases with increase in $P$ and the hypothesis testing threshold $\epsilon_{th}$ has a negative impact on $P_{md}$. This is due to the fact that $\epsilon_{th}$ extends the accepting range around actual position of legitimate AUV which makes some of the noisy estimates of malicious AUV appears in the accepting range of legitimate AUV. 

















==> Old_files/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This preliminary work studied physical layer authentication based on position of transmitting node. Position is estimated based on Time of Arrival (ToA) estimation for which best unbiased estimator was used. The distribution of uncertainty in estimation was derived. Further, to counter impersonation, binary hypothesis testing was used to classify the transmissions of transmitters into legitimate or malicious transmissions. The closed form expression for errors resulted from hypothesis testing were derived. We observed from simulation results that position can be used as device fingerprint for physical layer authentication. The follow up future work will counter mobility of legitimate AUV for investigation.

==> Old_files/giulio.tex <==


\section{Proposed Routing Mechanism}



In this section we present a novel routing mechanism that enables node to sink communication in the network described above. Firstly, we need to describe the topology of the network, which is dynamic over time. Then, we describe the process through which nodes maintain and spread information about the local topology introducing a congestion-avoidance mechanism. Finally, we describe the process through which each node selects a relay.

\subsection{Topology}
The network proposed in this work has a dynamic topology. Let $V$ be the set of nodes: $V = W \cup S \cup A$, namely, the underwater nodes, the surface nodes and the aerial nodes. 
For each node $u \in V$, we know the communication range $r_u$; moreover, let us define the node's state at time $t \in \mathbb
{Z}$ as the following tuple: 
\begin{equation}
    s_{u}(t) = \langle x_{u}(t), v_{u}(t), y_{u}(t), ?\rangle
\end{equation}

Considering the states of a node over time, we can describe its motion in a 3D space, where $x_{u}(t)$ represents the current coordinate of the node at time $t$, $v_{u}(t)$ represents the speed at which the node is moving at time $t$, and $y_{u}(t)$ represents coordinate of the next way-point (or direction) towards which the node is moving at time $t$.


Based on this model, it is possible to predict the future trajectory of the node. 
We assume that the node moves at a constant speed along a straight line without obstacles towards its next way-point. 
Note that the assumption of no obstacles in the environment is reasonable due to the fact that we are deploying the network in a marine environment.\todo{are we sure?} 
Given such assumption, at any given time $t$ and each time interval $\Delta t$,  we can compute the expected position at time $t + \Delta t$ of each node.
\begin{equation}
    x_{u}(t + \Delta t) = 
    \begin{cases}
    x_{u}(t) + x'_{u}(t) \Delta t & \text{if} \\
    y_{u}(t) & \text{otherwise}
    \end{cases}
\end{equation}

\todo{controlla formula, qui ci serve che $x_u(t + \Delta t)$ sia un punto sulla retta che congiunge x(t) e y(t). se lo spostamento è maggiore della distanza tra x e y allora questo punto è y altrimenti è a tale distanza da x }

This state formulation if applicable to both fixed and mobile nodes. Indeed, if a node is fixed, its speed is 0 and its coordinate never changes.

\todo{Assumption of connectivity over time, check}

%where: $x_{\psi}(t) \in \bathbb{R}^3$ is the coordinate of node ${\psi}$ at time $t$, $v_{\psi}(t) \in \bathbb{R}^+$ is the speed at which ${\psi}$ is moving, $y_{\psi}(t) \in \bathbb{R}^3$ is the next way-point (i.e., the direction towards $\psi$ is moving at time $t$).


\subsection{Network setup}
To being able to select a relay, each node has to be aware of which are the nodes in its communication range. To do so, we envisage a mechanism that allows nodes to set up and maintain forwarding tables.
Each node can enter the network broadcasting an \textit{hello packet}. Each node in the communication range which receives the hello packet stores  in its forwarding table node's state information contained in the hello packet. Each node can also decide to temporarily, or permanently, leave the network broadcasting a \textit{goodbye packet}. Each node should take this decision autonomously considering 
%its residual energy and 
the expected congestion considering its neighbourhood at a given time.

In the following we will describe in more details the hello packets, the forwarding table, the goodbye packets and the process through which a node decide whether to broadcast or not a goodbye packet. 

\subsubsection{Hello packet}
The \textit{hello packets} are used to signal node's availability and to exchange information between neighbours. Given a node $u$, the information contained are: (i) \textit{current position} $x_u(t)$ that express the 3-dimensional position of each node in the area, (ii) \textit{current speed} $v_u(t)$ that describe the instant speed at which the node is moving, (iii) \textit{next way-point} $y_u(t)$, namely, the next point in the node's trajectory if the node is mobile, (iv) \textit{buffer occupancy} that points out the current buffer occupation. 
\todo{forse ridondante, pensiamoci}
The node transmit in broadcast the hello packets periodically.

\todo{GIULIO riscrivere}
Let $t_0$ be the time at which the last hello packet has been sent, and let $t_1$ be the time at which the new packet has to be sent.


%Each node transmit a new hello packets if one of the following condition holds: i) , and let $\delta_{hello}$ be the maximum time a node can wait before broadcasting a new hello packet. Then, $t_1\le t_0 + \delta_{hello$;
 


Let us define $\delta_{hello}$ as the maximum time a node can wait before broadcasting a new hello packet. To deal with diverse mobilities of nodes \todo{(and maybe also other stuff)}, a node must send a new hello packet also whenever its state changes significantly from the last hello packet sent.

Thus let $t$ be the time at which $u$ has sent its last hello packet, $t' = min(\{\delta_{hello}\} \cup \{t'' : |s_u(t) - s_u(t'')| > \lambda \})$, where $\lambda$ is a threshold indicating the maximum change between two states before sending again the hello packet is necessary.
\todo{GIULIO fine}


\subsubsection{Neighbourhood}
The neighbourhood of a given node is computed using the hello packets received and then filtering out nodes that are not suitable to be selected as relays. The criteria we set up to exclude a node from the neighborhood are: \textit{age of information}, \textit{distance from the sender node}, \textit{belonging layer}. 
%Our goal is to exclude nodes with old information, that are too far to have a reliable connection quality,  denying the possibility to pass through the underwater layer once the data goes to the surface layer
The set of neighbours $N(\psi, t)$ of a node $\psi$ at time $t$ is defined using Equation \ref{eq:neghset}
    \todo{insert age of information condition for packets in eq \ref{eq:neghset}, modify u and place instead $\overline{\psi}$}
\begin{equation}
    N(\psi, t) = \{ u \in \Psi |\quad ||x_u(t) - x_{\psi}(t)|| < \sigma \wedge \psi \in S \cup A \rightarrow u \notin W \} 
    \label{eq:neghset}
\end{equation}
\todo{Insert details about equation 18}

\subsubsection{Goodbye packet}
Our network have to be efficient, for these reasons it is useful to manage congestion, avoiding packet loss and re-transmissions. To do that we include a control mechanism to forecast buffer saturation in a pre-defined temporal horizon. Given a node $u$ we define as $b_{u}(t)$ the buffer occupancy of the node $u$ at time $t$. We estimate $\Delta$ as the remaining time before buffer saturation \todo{add here}.
If the estimation $\Delta$ is below a certain threshold the node $u$ start sending in broadcast \textit{goodbye packets} telling the neighbours to exclude $u$ from the forwarding table.

\subsubsection{Table update}
\todo{Check if it can be included above}
Since we are modeling a protocol aimed at hybrid-mobility  networks (both static and mobile nodes) it is necessary to keep this table updated both to tackle node mobility and node availability. Thus, each entry has an expiration date that is updated each time the node receives a new hello packet from the node that corresponds to the entry. Moreover, the new state may change the goodness of the relay, requiring to reorder such entry in the table. To make this mechanism works, it is necessary that every node periodically sends a new hello packet containing its state. 

\subsection{Relay selection}
\todo{Make an example figure about the selection}
Whenever a node needs to transmit data, it may need to select the next hop so as to reach the ground station. 
We propose two selection methods: \textit{backbone relay selection}, and \textit{bubble relay selection}.

\paragraph{Backbone relay selection}: this mechanism is meant to be implemented in fixed wing UAVs, which constitute the top layer of the network topology. Once packets reached these nodes they should be forwarded only to other fixed wing UAVs or directly to the ground station. Note that this is possible due to the high-power long-range transmitter that this type of UAVs can be equipped with. Therefore, the relay selection is either the top layer node with the greatest advancement towards the ground station, or the ground station itself if it is in the communication range.

\paragraph{Bubble relay selection}: this mechanism has as objective of bringing the packets to the top layer of the network topology. Thus, each node selects the node in its neighbourhood with the greatest advancement towards the sky (i.e., the z axis). As a tie breaking rule the node with the greatest advancement towards the ground station is picked as a relay.
\todo{another TBR may be congestion avoidance}






==> bubble_routing_relay_selection.tex <==
\setlength{\textfloatsep}{4pt}% Remove \textfloatsep
\begin{algorithm}[t]
{

\footnotesize


\SetAlgoCaptionSeparator{:}
\KwIn{A set of nodes $R_u \subset V$ containing all the $u$ neighbours', the ground station $\Psi$ } 
\KwOut{A node $relay$ selected as relay}

\vspace{.2cm}
$R_u(t) \leftarrow \emptyset$\\
\For{$w \in N_u(t)$} {

    %If {$age(w) \leq \gamma $ \textbf{and} $||p_u(t) - p_w(t)|| < \sigma$ \textbf{and} $u \in S \cup A \rightarrow w \notin W$} {
    \If {$age(w) \leq \gamma $} {
       $R_u(t) \leftarrow R_u(t) \cup w$\\
        }
   
    }
$relay \leftarrow \emptyset$\\
$max \leftarrow 0$\\


\For{$w \in R_u(t)$} {

    $adv \leftarrow p_w(t).z - p_u(t).z$

    \If {$adv > max$} {
        $relay \leftarrow \{w\}$\\
    } 
    \Else {\If{$adv == max$}{
        $relay \leftarrow relay \cup \{w\}$\\
    }}
}
\If{$|relay| > 1$} {
    \textbf{return} $ \argmax_{w \in relay} ||p_\Psi - p_w(t + \Delta t)||$

}

\textbf{return} $relay$
}
\caption{Bubble Routing Relay Selection}
\label{algo:main}
\end{algorithm} 
